XChainWatcher: Monitoring and Identifying Attacks in Cross-Chain Bridges

Cross-chain bridges are a type of middleware for blockchain interoperability that supports the transfer of assets and data across blockchains. However, several of these bridges have vulnerabilities that have caused 3.2 billion dollars in losses since May 2021. Some studies have revealed the existence of these vulnerabilities, but there is little quantitative research available, and there are no safeguard mechanisms to protect bridges from such attacks. Furthermore, no studies are available on the practices of cross-chain bridges that can cause financial losses. We propose \toolName~(Cross-Chain Watcher), a modular and extensible logic-driven anomaly detector for cross-chain bridges. It operates in three main phases: (1) decoding events and transactions from multiple blockchains, (2) building logic relations from the extracted data, and (3) evaluating these relations against a set of detection rules. Using \toolName, we analyze data from two previously attacked bridges: the Ronin and Nomad bridges. \toolName~was able to successfully identify the transactions that led to losses of \$611M and \$190M (USD) and surpassed the results obtained by a reputable security firm in the latter. We not only uncover successful attacks, but also reveal other anomalies, such as 37 cross-chain transactions (\CCTX) that these bridges should not have accepted, failed attempts to exploit Nomad, over \$7.8M worth of tokens locked on one chain but never released on Ethereum, and \$200K lost by users due to inadequate interaction with bridges. We provide the first open dataset of 81,000 \CCTXS~across three blockchains, capturing more than \$4.2B in token transfers.

==> listings/listing-datalog-example.tex <==
\lstset{style=datalog}

\begin{lstlisting}[language=Datalog, caption={A cross-chain rule written in Datalog for the basic scenario of a cross-chain asset transfer.}, label={listing:datalog_example}]
ValidCCTX_Rule1(asset_id, tx_hash_A, tx_hash_B) :-
    Transaction(A, tx_hash_A, timestamp_tx_a),
    Transaction(B, tx_hash_B, timestamp_tx_b),
    LockAsset(asset_id, tx_hash_A),
    MintAsset(asset_id, tx_hash_B),
    timestamp_tx_b > timestamp_tx_a + (*@$\mathcal{\delta}$@*)
\end{lstlisting}

%\mpc{esta caption parecia-me errada -- The standardized signature of events emitted by the bridge contract once tokens are deposited.}

==> tables/latencies.tex <==
\setlength{\tabcolsep}{4.5pt} % Default value: 6pt

\begin{table}[ht]
\centering
\footnotesize
\rowcolors{2}{gray!10}{white}

\caption{Summary of CCTXs prior to attacks, including value transferred and latency metrics (in seconds).}
\begin{tabular}{lrrrr}
\toprule
 & \multicolumn{2}{c}{Nomad Bridge} & \multicolumn{2}{c}{Ronin Bridge} \\
\cmidrule(rl){2-3} \cmidrule(rl){4-5} 

 & Deposits & Withdrawals & Deposits  & Withdrawals \\ \midrule
 
Number of CCTXs & \sizecctxdepositslatencyNomad & \sizecctxwithdrawalslatencyNomad & \sizecctxdepositslatencyRonin & \sizecctxwithdrawalslatencyRonin  \\
Min Latency & \mincctxdepositslatencyNomad & \mincctxwithdrawalslatencyNomad & \mincctxdepositslatencyRonin & \mincctxwithdrawalslatencyRonin  \\
Max Latency & \maxcctxdepositslatencyNomad & \maxcctxwithdrawalslatencyNomad & \maxcctxdepositslatencyRonin & \maxcctxwithdrawalslatencyRonin  \\
Avg Latency & \avgcctxdepositslatencyNomad & \avgcctxwithdrawalslatencyNomad & \avgcctxdepositslatencyRonin & \avgcctxwithdrawalslatencyRonin  \\
Std Dev Latency & \stdcctxdepositslatencyNomad & \stdcctxwithdrawalslatencyNomad & \stdcctxdepositslatencyRonin & \stdcctxwithdrawalslatencyRonin  \\
Median Latency & \mediancctxdepositslatencyNomad & \mediancctxwithdrawalslatencyNomad & \mediancctxdepositslatencyRonin & \mediancctxwithdrawalslatencyRonin  \\
\hdashline
\addlinespace[0.05cm]
\rowcolor{gray!10}Total Value (USD) & \textbf{\$\totalvaluedepositsbeforeattackNomad M} & \textbf{\$\totalvaluewithdrawalsbeforeattackNomad M} & \textbf{\$\totalvaluedepositsbeforeattackRonin M} & \textbf{\$\totalvaluewithdrawalsbeforeattackRonin M}  \\ \bottomrule
\end{tabular}\label{table: cctx_latencies}
\begin{tablenotes}
\footnotesize
\item \textit{Note:} ``Lat'' means Latency. %Also, we only include cctxs in which all events in all chains completed before the attacks to remove the influence of bridge pauses in the values presented.
\end{tablenotes}
\end{table}

